Towards Practical Lipschitz Bandits

Stochastic Lipschitz bandit algorithms balance exploration and exploitation, and have been used for a variety of important task domains. In this paper, we present a framework for Lipschitz bandit methods that adaptively learns partitions of context- and arm-space. Due to this flexibility, the algorithm is able to efficiently optimize rewards and minimize regret, by focusing on the portions of the space that are most relevant. In our analysis, we link tree-based methods to Gaussian processes. In light of our analysis, we design a novel hierarchical Bayesian model for Lipschitz bandit problems. Our experiments show that our algorithms can achieve state-of-the-art performance in challenging real-world tasks such as neural network hyperparameter tuning.

==> tex/app.tex <==
\section{Reproducibility Notes}

Major environment configuration for experiments in the paper: 

\begin{itemize}
    \item Python 3.6.4
    \item TensorFlow (GPU version) 1.15 
    \item Hardware for wallclock time experiments in Figure \ref{fig:tune-nn-mnist}: Dell Precision T3620
    \begin{itemize}
        \item Processor: 6th Gen Intel Core i7-6700 (Quad Core 3.40GHz, 4.0Ghz Turbo, 8MB)
        \item Memory: 32GB (4x8GB) 2133MHz DDR4 Non-ECC
        \item Video Card: NVIDIA Quadro K620, 2GB
        \item HDD: 256GB SATA Class 20 Solid State Drive. 
    \end{itemize} 
    % \item 
\end{itemize} 

Code is available at (anonymous file sharing): \url{https://drive.google.com/open?id=1IVvwaQZ8GRffcYLUH4rZbfLVUtTXBAxS}. 

\textbf{Note}: Users need to install the scikit-learn package provided in the above link in order to run the scripts for the TreeUCB algorithm. 

==> tex/experiments.tex <==
% \vspace{-5pt}
% \section{Implementation and Experiments} \label{sec:exp}

% \vspace{-8pt}
% \subsection{Application to Neural Network tuning}
% \label{sec:tune-nn}
% % \vspace{-5pt}
% \textbf{\emph{Experimental design}}: 
% Given fixed training and validation sets, the validation accuracy of a neural network can be viewed as a noisy function of hyperparameters. Typical hyperparameters for tuning include the network architecture, learning rate, training iterations, etc. The number of training iterations is itself a hyperparameter, but it is a special one -- training accuracy tends to increase with the number of training iterations, and we may only care about the performance at a large enough training iteration. 
% In addition, some tuning methods have a special scheme to leverage the training iterations as a special dimension, while some do not. 
% %Because of this, we may tune the number of training iterations together with other hyperparameters, or leverage the number of training iterations as a special dimension. 
% Therefore we divide the experiments into two settings: A) the algorithms are agnostic to the training resource and thus 
% %treat the number of training iterations in the same way as they treat all other hyperparameters, and 
% tune the training iterations together with all other hyperparameters; B) the algorithms leverage the number of training iterations as a special dimension using their own schemes (if it has one). We will refer to these two settings as \textit{setting A} and \textit{setting B} from now on; we compare TUCB against other methods in Setting A, and compare CTUCB against other methods in Setting B. %Some of the state-of-the-art tuning methods explicitly leverage number of training iterations as a special dimension, while some do not. 
%This suggests that comparing the methods in these two different settings better reflects their tuning performance.

%One problem for tuning a neural network is that we not only want to minimize the number of queries we make, we also want to restrict the average computational resources needed for each query. We use the number of epochs (or, iterations) needed as the measure of computational resources needed. At smaller epochs, the validation accuracy tends to be smaller; at larger epochs, the validation accuracy tends to be larger. Formally, we factorize out the resource dimension from the rest of hyperparameter configurations, and formulate this problem as follows: for a fixed dataset (training and validation), and fixed seeds for all randomness, the validation accuracy of a neural network on this dataset can be defined as a function of hyperparameter configuration and the training resource (number of training epochs), 
%\begin{align}
%h : \mathcal{Z} \times \mathcal{A} \rightarrow [0,1] \label{eq:nn-loss}
%\end{align}
%where $\mathcal{Z}$ is the training resource dimension (training epochs) and $\mathcal{A}$ is the rest of the hyperparameter configurations space. 

%\emph{\textbf{Regularization along resource}}. 
%This problem is special since we want to limit the resource usage. This can be achieved by adding a term that gives a bonus to configurations whose resource usage is small. For a configuration  $ (z, a) $ at time $t$, we add a correction term $ \mathcal{B} (z, t) $ to the UCB. In principle, the UCB gets a bonus when the resource usage is small, and this bonus decreases as time $t$ increases. In addition, as the training epoch increases, the validation accuracy converges. Therefore, on a local scale, the Lipschitz constant decreases as the training epoch increases. As stated in Algorithm \ref{alg:contextual-bandit}, the confidence term is $\beta_t \sqrt{ \frac{1}{n_{t-1} (z, a)} } $ with $\beta_t = \left( \alpha c + \sqrt{ \left( \frac{1}{2} + 2 s^2 \right) \left( \log t + \log 2 \right) } \right)$. Instead of using the global Lipschitz constant $c$, we use $\mathcal{C} ( z ) $ to model the Lipschitz constant. Since  neural networks converge as training resource increases, $\mathcal{C} ( z ) $ is positive and decreases with $z$. 

%Thus we pick $(z_t, a_t) \in \arg \max_{(z, a)} \left\{ m_{t-1}(z, a) + v_1  \sqrt{ \frac{ \log t }{n_{t-1} (z, a)} } + v_2 \frac{1}{zt} \right\} $ at step $t$. This algorithm is summarized in Algorithm \ref{alg:regularize}. 

% \emph{\textbf{Using training iterations as contextual information}}. 
%\textcolor{red}{Won't this paragraph serve as an explanation of how to use the training iterations as a special one?}
% Context is usually observed from the environment, but in this case, we are able to choose it. We let CTUCB start with a small number of training iterations and progressively increase the number of iterations. By doing this, CTUCB can use information obtained at smaller iterations (cheaper to obtain) to help infer the performance at larger iterations (more expensive to obtain). This assumes that a configuration that is good at smaller iterations tends to be good at larger iterations as well, which tended to be true in practice for our experiments. 
% \textcolor{red}{ While the number of training iterations can be considered as a hyperparameter for tuning (as in Setting A), it is also very special: (i) with all (other) hyperparameters fixed, the validation accuracy tends to increase with the training iterations; (ii) the larger the training iteration, the more expensive the evaluation of a configuration is. Therefore, in Setting B, CTUCB does not consider training iterations as a hyperparameter for tuning. Instead, we leverage this information in the following way: we let CTUCB see it as (part of) the contextual information. We let CTUCB start with a small number of training iterations and progressively increase the number of iterations. By doing this, CTUCB can use information obtained at smaller iterations (cheaper to obtain) to help infer the performance at larger iterations (more expensive to obtain). This assumes that a configuration that is good at smaller iterations tends to be good at larger iterations as well, which tended to be true in practice for our experiments. 
% Context is usually observed from the environment, but in this case, we are able to choose it.
% Unlike traditional contextual bandit problems, we choose this context (the number of training iterations), instead of observing it from the environment. } 
%In short, CTUCB leverages training iterations by using it as contextual information in \textit{setting B}. 
% As shown in Figures \ref{fig:mlp-mnist}, \ref{fig:cnn-svhn} and \ref{fig:cnn-cifar} by using training iterations as the contextual information, CTUCB can outperform existing state-of-the-art methods. 
%\textcolor{red}{do you mean setting A? - It's setting B. I'm answering this by more clarification on the definition of setting A and B.}

% \emph{\textbf{Modeling the Lipschitz constant with the number of training iterations.}} 
% In \textit{setting B}, for a hyperparameter configuration $a$, as the training iteration $z$ increases, the validation accuracy converges. Therefore, on a local scale, the Lipschitz constant decreases as the training iteration (epoch) increases. As stated in Algorithm \ref{alg:contextual-bandit}, the confidence coefficient is $\beta_t \sqrt{ \frac{1}{n_{t-1} (z, a)} } $ with $\beta_t = \BETAt.$ Instead of using the global Lipschitz constant $c$, we can use $\mathcal{C} ( z ) $ to model the local Lipschitz constant if there is enough prior knowledge. Since neural networks converge as training resource increases, $\mathcal{C} ( z ) $ should be positive and decreases with $z$. 

%Both Algorithm \ref{alg:tucb} and \ref{alg:ctucb} need hyperparameters as inputs. Nonetheless, both algorithms are fairly robust to the choice of those hyperparameters, as we will see in Section \ref{sec:exp}. In Section \ref{sec:exp}, we use $\mathcal{C} (z ) = z^{v_3}$ where $v_3 \le 0$ is a constant hyperparameter. Recommendations for choosing these hyperparameters are also in Section \ref{sec:exp}. 

% in the following sense: 
%%
%\item We want to limit resource usage. %We can achieve this by model the resource as the context, and let the context arrives in a certain way, so that we evaluate $h$ more often at smaller epochs. 
%\item As the training epoch increases, the validation accuracy converges. %Therefore, on a local scale, the Lipschitz constant decreases as the training epoch increases. As stated in Algorithm \ref{alg:contextual-bandit}, the upper confidence bound is $\left\{ m_{t-1}(z_t, a) + \beta_t \sqrt{ \frac{1}{n_{t-1} (z_t, a)} } \right\} $ with $\beta_t = \left( \alpha c + \sqrt{  \left( \frac{1}{2} + 2 s^2 \right) \left( \log t + \log 2 \right) } \right)$. Here $c$ is the global Lipschitz constant. Thus with all other variables fixed, $\beta_t$ should decrease as $t$ increases.
%\end{enumerate}
%The above two items can be stressed using the following 

%Taking this into consideration, we first define a epoch range $[z_0, z_*]$ and a total number of queries $N \ge 2$. We select the epochs $z_1, z_2, \cdots z_N \in [z_0, z_*]$ such that $\log z_{i+1} - \log z_i = \frac{\log z_* - \log z_0}{ N - 1 } $, $z_1 = z_0$ and $z_N = z_*$. In words, $z_1, z_2, \cdots, z_N$ is distributed along $[z_0, z_*]$ on a log scale. Second, the upper confidence bound is computed as $ \left\{ m_{t-1}(z_t, a) + \beta_t^\prime \sqrt{ \frac{1}{n_{t-1} (z_t, a)} } \right\} $ where $\beta_t^\prime = v_1 z_t^{-v_3} + v_2 \sqrt{ \log t }$ and $v_1, v_2, v_3 > 0$ are parameters that trade off exploration and exploitation. Although Algorithm \ref{alg:context-tree} itself has parameters to choose, the performance of Algorithm \ref{alg:context-tree} is robust to the choice of $v_1, v_2, v_3$. A detailed study of this issue is in Section \ref{experiment}. 

%In this section, we study TreeUCB (TUCB) and Contextual TreeUCB (CTUCB) empirically. In all experiments, we set $\mathcal{C} (z) = z ^ {v_3}$ where $v_3 \le 0$ is an input hyperparameter of TUCB and CTUCB. We first study the behavior of these algorithms when $v_1, v_2, v_3, \eta$ change on a synthetic function. %In fact, Algorithms \ref{alg:regularize} and \ref{alg:context-tree} are insensitive to most of the parameters. 
% \subsection{Synthetic function}

% A variation of the H\"older's table function:
% \begin{align}
% f (a_1, a_2, z) = \max \left( 0.25,  \left( \frac{11}{60} - \frac{1}{6 z} \right) \sin a_1 \cos a_2 \exp \left( \left| 1 -  \frac{ \sqrt{ a_1^2 + a_2^2 } }{ 2 \pi}  \right| \right)  + \frac{1}{2} \right) ,
% \end{align}
% with $a_1, a_2 \in [-10, 10 ]$ and $z \in [ 1, 1000] $, is used to study Algorithm \ref{alg:tucb} and \ref{alg:ctucb}. This function is referred to as the z-H\"older function, and the function surfaces (when $z = 1$ and $z= 1000$) are in Figure \ref{fig:synthetic-function}. In the z-H\"older function, $z$ is the resource dimension. 

% \begin{figure}%
% \centering
% \subfloat[$z = 1$.]{\includegraphics[scale = 0.45]{./figures/fholder1.eps} }
% \subfloat[$z = 1000$.]{ \includegraphics[scale = 0.45]{./figures/fholder1000.eps} }\\
% %\subfloat[Third.]{ \includegraphics{./figures/fholder1.png}  }%
% \caption{The z-H\"older's function with $z = 1$ and $z=1000$. \label{fig:synthetic-function}}
% \end{figure}

% The range of the z-H\"older's function is within $[0.25,1]$.%, and the maximal value is approximately $0.98$. 
% By running TreeUCB and Contextual TreeUCB on the z-H\"older's function, we observe that TreeUCB and Contextual TreeUCB are insensitive to most choices of parameters. The results for TreeUCB and Contextual TreeUCB are summarized in Figure \ref{fig:tune-tucb} and \ref{fig:tune-ctucb}, respectively. 
% Based on the results in Figure \ref{fig:tune-tucb} and \ref{fig:tune-ctucb}. We make the following recommendation for choosing $\eta, v_1$, (and $v_2, v_3$). For both TUCB and CTUCB, we recommend setting $\eta$ to the same order as $0.001-0.0001$, $v_1$ to the same order as 0.1. For CTUCB, in general cases where the \textit{number of iterations} goes above $10^2$, we recommend setting $v_2$ to the same order as 1, and setting $v_3$ between -1 and -2. 

% \begin{figure}%tree_tune_ete_v1=02_resource
% \centering
% \subfloat[$v_1 = 0.2$.]{\includegraphics[scale = 0.45]{./figures/tree_tune_eta_v1=02.eps} }
% \subfloat[$v_1 = 0.2$.]{\includegraphics[scale = 0.45]{./figures/tree_tune_eta_v1=02_resource.eps} } \\
% \subfloat[$\eta = 0.001$.]{ \includegraphics[scale = 0.45]{./figures/tree_tune_v1_eta=0001.eps} }
% \subfloat[$\eta = 0.001$.]{ \includegraphics[scale = 0.45]{./figures/tree_tune_v1_eta=0001_resource.eps} }\\
% %\subfloat[Third.]{ \includegraphics{./figures/fholder1.png}  }%
% \caption{Results for TreeUCB (TUCB). Left column: the performance is measured by current best value obtained versus how many times we have queried the z-H\"older's function (number of trials); Right column: the performance is measured by current best value obtained versus how much resource are used. For $\eta$, large $\eta$ results in large leaf, and vice versa. As shown above, TUCB is not very sensitive to the choice of $\eta$ except when it is too large. We recommend setting $\eta$ to the same order as $0.001 - 0.0001$. For $v_1$, TreeUCB needs a non-zero $v_1$ to escape a local optimum, and is fairly robust to the choice of $v_1$. All line plots are averaged over 50 runs. \label{fig:tune-tucb}}
% \end{figure}

% \begin{figure}%
% \centering
% \subfloat[$v_1 = 0.4$, \newline $v_2 = 4, v_3 = -1$.]{\includegraphics[scale = 0.3]{./figures/tree_context_tune_eta_v1=04_v2=4_v3=-1.eps} }
% \subfloat[$v_1 = 0.4$, \newline $v_2 = 4, v_3 = -1$.]{\includegraphics[scale = 0.3]{./figures/tree_context_tune_eta_v1=04_v2=4_v3=-1_resource.eps} } 
% \subfloat[$\eta = 0.002, v_2 = 0$.]{\includegraphics[scale = 0.3]{./figures/tree_context_tune_v1_v2=0_v3=-1_eta=0002.eps} } \\
% \subfloat[$\eta = 0.002, v_2 = 0$.]{\includegraphics[scale = 0.3]{./figures/tree_context_tune_v1_v2=0_v3=-1_eta=0002_resource.eps} } 
% \subfloat[$\eta = 0.002$, \newline $v_1 = 0, v_3 = -2$.]{\includegraphics[scale = 0.3]{./figures/tree_context_tune_v2_v1=0_v3=-2_eta=0002.eps} }
% \subfloat[$\eta = 0.002$, \newline $v_1 = 0, v_3 = -2$.]{\includegraphics[scale = 0.3]{./figures/tree_context_tune_v2_v1=0_v3=-2_eta=0002_resource.eps} } \\
% \subfloat[$\eta = 0.001$, \newline $v_1 = 0, v_2 = 2$.]{\includegraphics[scale = 0.3]{./figures/tree_context_tune_v3_v1=02_v2=2_eta=0001.eps} }
% \subfloat[$\eta = 0.001$, \newline $v_1 = 0, v_2 = 2$.]{\includegraphics[scale = 0.3]{./figures/tree_context_tune_v3_v1=02_v2=2_eta=0001_resource.eps} } \\

% %\subfloat[Third.]{ \includegraphics{./figures/fholder1.png}  }% 
% \caption{Results for Contextual TreeUCB (CTUCB). (a), (c), (e), (g): the performance is measured by current best value obtained versus how many times we have queried the z-H\"older's function (number of trials); (b), (d), (f), (h): the performance is measured by current best value obtained versus how much resource are used. For $\eta$, large $\eta$ results in large leaf, and vice versa. For $\eta$, CTUCB is not very sensitive as long as $\eta$ is not too large. We recommend setting $\eta$ to the same order as $0.001 - 0.0001$. For $v_1$, CTUCB needs a non-zero $v_1$ to escape a local optimum, and is fairly robust to the choice of $v_1$. For $v_2$ and $v_3$, CTUCB is again fairly robust to the choice of $v_2$ and $v_3$ while non-zero $v_2, v_3$ improve the performance. When measured by resources used, Contextual TreeUCB converges much faster. All line plots are averaged aver 50 runs. \label{fig:tune-ctucb}}
% \end{figure}
% \vspace{-8pt}
\subsection{Experiments} \label{sec:exp-real}
% \vspace{-5pt}
In this section, we compare the performance of TUCB and CTUCB on the MNIST dataset, the SVHN dataset, and the CIFAR-10 dateset. In \textit{setting A} we compare SMAC, random search, TPE, Spearmint, Harmonica-r (Harmonica using random search as the base algorithm) and TUCB. In \textit{setting B}, we compare SMAC, random search, TPE, Spearmint, CTUCB, Hyperband and Harmonica-h (Harmonica using Hyperband as the base algorithm). In \textit{setting B}, CTUCB, Hyperband and Harmonica-h set the \textit{number of training iterations} using their own schemes, while the rest of the algorithms fix the \textit{number of training iterations} and tune the rest of the hyperparameters. In particular, CTUCB uses the number of training iterations as the contextual information. How we set the training iterations for CTUCB will be specified later. 
% \vspace{-5mm}
\subsubsection{MLP for MNIST}  
\label{sec:mlp-mnist}
% \vspace{-5pt}
In this section, we tune a simple Multi-Layer Perceptron (MLP) and compare TUCB and CTUCB with state-of-the-art methods. For TUCB, we use $\beta_t = v \sqrt{\log t}$, where $v$ is a hyperparameter of the tuning algorithm; and for CTUCB in tuning neural networks, we use $\beta_t = v_1 \sqrt{\log t} + v_2 z ^{v_3}$, where $z$ is the number of training iterations, and $v_2 z ^{v_3}$ models the local Lipschitz constant. In this case, $v_1$, $v_2$ and $v_3$ are all hyperparameters of the tuning algorithm. Although TUCB and CTUCB have their own hyperparameters, the performance of both TUCB and CTUCB are not sensitive to these hyperparameters. The architecture of this MLP is as follows: in the feed-forward direction, there are the \textit{input layer}, the \textit{fully connected hidden layer with dropout ensemble}, and then the \textit{output layer}. The hyperparameter search space is \textit{number of hidden neurons} (range $[10, 784 ]$), \textit{learning rate} ($[0.0001, 4 )$), \textit{dropout rate} ($[0.1, 0.9)$), \textit{batch size} ($[10, 500]$), \textit{number of iterations} ($[30, 243]$). In \textit{setting B}: All algorithms except for Hyperband, CTUCB, Harmonica-h always use 243 for the number of iterations. \footnote{We choose the number 243 so that it helps Hyperband avoid rounding using their example down-sampling rate 3.} Hyperband, CTUCB and Harmonica-h use their own specific mechanisms to alter \textit{number of iterations}. The results are shown in Figure \ref{fig:mlp-mnist}. For CTUCB in Setting B, we choose the training iterations $z_t$ so that
\begin{align*}
z_t &= 
\begin{cases}
\lfloor 1/ (1/30 - ( t \mod 33) ( 1/30 - 1/243) / 29 ) \rfloor, \\
\qquad \qquad \qquad \qquad \qquad \text{if } t \mod 33 < 30, \\
243, \quad \text{otherwise}. 
\end{cases}
\end{align*}

By setting $z_t$ this way, CTUCB repeatedly starts with small iterations and proceeds to larger iterations (and repeats). 
%This way, CTUCB uses the information collected in smaller iterations to help the decisions at larger iterations. 
As shown in Figure \ref{fig:mlp-mnist}, our methods find good configurations faster than other methods, in both Setting A and Setting B. 
%In Setting B, CTUCB on average reaches 0.96 accuracy within 120 seconds; and in Setting A, TUCB only reaches 0.96 accuracy within 120 seconds. Therefore, using Setting B gives us an advantage on the absolute scale. 
%In particular, in Setting A, TUCB reaches 0.9 accuracy using xx seconds, while the other methods reaches 0.9 using xx seconds; in Setting B, TUCB reaches 0.9 accuracy using xx seconds, while the second best method reaches 0.9 accuracy using xx seconds, and other methods on average reaches 0.9 accuracy using xx seconds. \footnote{We consider a method using 120 seconds to reach 0.9 accuracy if it does not reach 0.9 accuracy within 120 seconds.} }
% % \vspace{-10pt}

% \begin{figure}[H]
% \centering
% \includegraphics[scale = 0.3]{./figures/legends-3.png}  \\
% %\vspace{-10pt}
% \subfloat[Setting A.]{\includegraphics[scale = 0.37]{./figures/MNIST_non_contextual.png} }  \hspace{2.5cm}
% \subfloat[Setting B.]{\includegraphics[scale = 0.37]{./figures/MNIST_contextual.png} }
% %\vspace{-6pt}
% \caption{Current best validation accuracy against wall clock time on MNIST. \textit{Left:} Setting A. TUCB: $v = 0.1, \eta = 0.0001$. \textit{Right:} Setting B. CTUCB: $ v_1 = 0.1, v_2 = 1, v_3 = -2, \eta = 0.0001$. The results for all methods are averaged over 10 runs. As is shown in the plots, TUCB and CTUCB find good configurations faster than other methods for the experiments in Section \ref{sec:mlp-mnist}. %In this set of experiments, wall clock time is a measure of training resource. 
% \label{fig:mlp-mnist} } 
% %\vspace{-10pt}
% \end{figure}


% \subsection{AlexNet CNN for SVHN}
% In this section, we tune an AlexNet-type \cite{krizhevsky2012imagenet} CNN \cite{lecun1998gradient} for the SVHN dataset and compare TUCB and CTUCB with state-of-the-art methods. The architecture of this CNN and the corresponding hyperparameters are summarized in Table \ref{tab:svhn-arch} and \ref{tab:svhn-params}. The results are shown below in Figure \ref{fig:cnn-svhn}. For CTUCB in Setting B, we pick context $z_t$ (the training iterations) so that 
% \begin{align*}
% z_t &= 
% \begin{cases}
% \lfloor 1/ (1/100 - ( t \mod 34) ( 1/100 - 1/1500) / 29 ) \rfloor, \\ 
% \qquad \qquad \qquad \qquad \qquad \text{if } t \mod 34 < 30, \\
% 1500, \quad \text{otherwise}. 
% \end{cases}
% \end{align*}
% By setting $z_t$ in this way, CTUCB starts with small training iteration and progressively increases it (and repeats).
% %CTUCB saves resources by using information at small iterations to help decisions at larger iterations. The results are summarized in Figure \ref{fig:cnn-svhn}. 
% In this set of experiments, TUCB and CTUCB usually find good configurations at least as fast as other methods. %In particular, in Setting B, Hyperband ties CTUCB and both methods are better than the rest. %In particular, TUCB reaches 0.8 accuracy within xx total iterations in Setting A, while other methods on average use yy iterations to reach the same accuracy; and CTUCB reaches 0.8 accuracy within xx total iterations in Setting B, while other methods on average use yy iterations to reach the same accuracy. \footnote{}

% \begin{figure}[H]% 
% \centering
% \includegraphics[scale = 0.3]{./figures/legends-3} \\
% \subfloat[Setting A.]{\includegraphics[scale = 0.37]{./figures/SVHN_non_contextual} } \hspace{2.5cm}
% % \vspace{-8pt}
% \subfloat[Setting B.]{\includegraphics[scale = 0.37]{./figures/SVHN_contextual} }
% % \vspace{-5pt}
% \caption{Current best validation accuracy against total training iterations used on SVHN. \textit{Left:} Setting A. TUCB: $ v_1 = 0.1, \eta = 0.001$.  \textit{Right:} Setting B. CTUCB: $ v_1 = 0.1, v_2 = 1, v_3 = -2, \eta = 0.001$. All other algorithms use default setting. The results for all methods are averaged over 5 runs. For all methods, if a configuration diverged (having a diverging cross-entropy loss), its chosen number of iterations is used as the training resource used, even if the training terminates early because of the diverging cost. \label{fig:cnn-svhn}}
% \vspace{-10pt}
% \end{figure} 

% \begin{figure}[H]% 
% \centering
% \includegraphics[scale = 0.35]{./figures/legends-3.png} \\
% %\vspace{-10pt}
% \subfloat[Setting A.]{\includegraphics[scale = 0.37]{./figures/CIFAR_non_contextual.png} } \hspace{2.5cm}
% \subfloat[Setting B.]{\includegraphics[scale = 0.37]{./figures/CIFAR_contextual.png} }
% %\vspace{-6pt}
% \caption{Plot of current best validation accuracy versus total training iterations used on CIFAR. \textit{Left:} Setting A. TUCB: $ v_1 = 0.1, \eta = 0.0001$.  \textit{Right:} Setting B. CTUCB: $ v_1 = 0.1, v_2 = 1, v_3 = -2, \eta = 0.0001$. All other algorithms use default setting. The results for all methods are averaged over 5 runs. As is shown in the plots, TUCB and CTUCB find good configurations faster than other methods most of the time. In Setting A, Harmonica performed slightly better in early stage, but TUCB achieves a higher final accuracy. In Setting B, Hyperband ties CTUCB and both Hyperband and CTUCB are better than other methods. For all methods, if a configuration diverged (having a diverging cross-entropy loss), its chosen number of iterations is still used as the training resource used. For all methods, if a configuration diverged (having a diverging cross-entropy loss), its chosen number of iterations is used as the training resource used, even if the training terminates early because of the diverging cost. %In Setting B, CTUCB reaches 0.76 accuracy within 45,000 iterations, and in Setting A, TUCB only reaches 0.75 accuracy within 45,000 iterations. Therefore, using Setting B gives us an advantage on the absolute scale.
% %In this set of experiments, the number of iterations taken is used has a measure of training resource. 
% \label{fig:cnn-cifar}}
% %\vspace{-10pt}
% \end{figure} 

% % \begin{tabular}{ c c c }
% % Layer & Hyperparameters & values \\ \hline 
% % \multirow{4}{*}{  Conv1  }  & conv1-kernel-size & $$  \\
% % &  conv1-number-of-channels & 200 \\
% % &  conv1-stride-size & (1,1) \\
% % &  conv1-padding & ``same'' \\
% %  Conv3 &   \\
% %  Dense & 
% % \end{tabular} 

% \begin{table}[H]
% \centering
% \vspace{1.5cm}
% \subfloat[][CNN architecture for SVHN. A value with * means that this parameter is tuned, and the batch-normalization layer uses all Tensorflow's default setting. \label{tab:svhn-arch} ]{
% \begin{tabular}{ c c c }
% Layer & Hyperparameters & values \\ \hline \hline
% \multirow{4}{*}{  Conv1  }  & conv1-kernel-size & *  \\
% &  conv1-number-of-channels & 200 \\
% &  conv1-stride-size & (1,1) \\
% &  conv1-padding & ``same'' \\ \hline
% \multirow{3}{*}{  MaxPooling1  }  & pooling1-size & (3,3)  \\
% &  pooling1-stride & (1,1) \\
% &  pooling1-padding & ``same'' \\ \hline
% \multirow{4}{*}{  Conv2  }  & conv2-kernel-size & *  \\
% &  conv2-number-of-channels & 200 \\
% &  conv2-stride-size & (1,1) \\
% &  conv2-padding & ``same'' \\ \hline
% \multirow{3}{*}{  MaxPooling2  }  & pooling2-size & (3,3)  \\
% &  pooling2-stride & (2,2) \\
% &  pooling2-padding & ``same'' \\ \hline
% \multirow{4}{*}{  Conv3  }  & conv3-kernel-size & (3,3)  \\
% &  conv3-number-of-channels & 200 \\
% &  conv3-stride-size & (1,1) \\
% &  conv3-padding & ``same'' \\ \hline
% \multirow{3}{*}{  AvgPooling3  }  & pooling3-size & (3,3)  \\
% &  pooling3-stride & (1,1) \\
% &  pooling3-padding & ``same'' \\ \hline
%  \multirow{3}{*}{  Dense  }  & batch-normalization & default \\ 
%  & number-of-hidden-units & 512 \\ 
%  & dropout-rate & 0.5 \\ \hline
% \end{tabular}
% } \\
% % \hfill
% \vspace{1.5cm}
% \subfloat[][Hyperparameter search space. $\beta_1$ and $\beta_2$ are parameters for the Adamoptimizer. The learning rate is discretized in the following way: from 1e-6 to is 1 (including the end points), we log-space the learning rate into 50 points, and from 1.08 to 5 (including the end points) we linear-space the learning rate into 49 points. \label{tab:svhn-params}]{
% \begin{tabular}{ c c c }
% Hyperparameters & Range  \\ \hline \hline 
% conv1-kernel-size & $\{1,2,\cdots,7\}$ \\ \hline 
% conv2-kernel-size & $\{1,2,\cdots,7\}$ \\ \hline 
% $\beta_1$ & $\{0 , 0.05 ,  \cdots, 1 \}$  \\ \hline 
% $\beta_2$ & $\{0 , 0.05 ,  \cdots, 1 |$  \\ \hline 
% learning-rate & 1e-6 to 5 \\ \hline 
% \makecell{training-iteration \\ (only for Setting A) } & $\{300,400, \cdots,1500\}$ \\ \hline
% \end{tabular}
% }
% % \vspace{-8pt}
% \caption{Settings for the SVHN experiments.}
% % \vspace{-10pt}
% \end{table}

% \newpage~
% % \vspace{-5pt}
% \subsubsection{AlexNet CNN for CIFAR-10}
% % \vspace{-5pt}
% \label{sec:cifar}
% In this section, we tune an AlexNet-type \cite{krizhevsky2012imagenet} CNN \cite{lecun1998gradient} for the CIFAR-10 dataset \cite{krizhevsky2009learning} and compare TUCB and CTUCB with state-of-the-art methods. The architecture of this CNN and the corresponding hyperparameters are summarized in Table \ref{tab:cifar-arch} and \ref{tab:cifar-params}. The results are shown below in Figure \ref{fig:cnn-cifar}. For CTUCB in Setting B, we pick context $z_t$ (the training iterations) so that CTUCB increases the number of training iterations in exactly the same way as Hyperband. Hyperband and CTUCB increase the number of training as shown in Table \ref{tab:cifar-resouce}. This progression of training iterations is determined by Hyperband's hyperparameters. Please refer to the Hyperband paper \cite{li2016hyperband} for more details on how Hyperband selects training resources. 

% % \newpage~\newpage~
% \begin{table}[H]
% \centering
% \vspace{3cm}
% \subfloat[][CNN architecture for CIFAR-10. A value with * means that this parameter is tuned, and the batch-normalization layer uses all Tensorflow's default setting. \label{tab:cifar-arch} ]{
% \begin{tabular}{ c c c }
% Layer & Hyperparameters & values \\ \hline \hline
% \multirow{4}{*}{  Conv1  }  & conv1-kernel-size & *  \\
% &  conv1-number-of-channels & 200 \\
% &  conv1-stride-size & (1,1) \\
% &  conv1-padding & ``same'' \\ \hline
% \multirow{3}{*}{  MaxPooling1  }  & pooling1-size & *  \\
% &  pooling1-stride & (1,1) \\
% &  pooling1-padding & ``same'' \\ \hline
% \multirow{4}{*}{  Conv2  }  & conv2-kernel-size & *  \\
% &  conv2-number-of-channels & 200 \\
% &  conv2-stride-size & (1,1) \\
% &  conv2-padding & ``same'' \\ \hline
% \multirow{3}{*}{  MaxPooling2  }  & pooling2-size & *  \\
% &  pooling2-stride & (2,2) \\
% &  pooling2-padding & ``same'' \\ \hline
% \multirow{4}{*}{  Conv3  }  & conv3-kernel-size & *  \\
% &  conv3-number-of-channels & 200 \\
% &  conv3-stride-size & (1,1) \\
% &  conv3-padding & ``same'' \\ \hline
% \multirow{3}{*}{  AvgPooling3  }  & pooling3-size & *  \\
% &  pooling3-stride & (1,1) \\
% &  pooling3-padding & ``same'' \\ \hline
%  \multirow{3}{*}{  Dense  }  & batch-normalization & default \\ 
%  & number-of-hidden-units & 512 \\ 
%  & dropout-rate & 0.5 \\ \hline
% \end{tabular}
% } \hfill
% \subfloat[][Hyperparameter search space. $\beta_1$ and $\beta_2$ are parameters for the Adamoptimizer. The learning rate is discretized in the following way: from 1e-6 to is 1 (including the end points), we log-space the learning rate into 50 points, and from 1.08 to 5 (including the end points) we linear-space the learning rate into 49 points. The learning-rate-reduction parameter is how many times the learning rate is going to be reduced by a factor of 10. For example, if the total training iteration is 200, the learning-rate is 1e-6, and the learning-rate-reduction is 1, then for the first 100 iteration the learning rate is 1e-6, and the for last 100 iterations the learning rate is 1e-7. \label{tab:cifar-params}]{
% \begin{tabular}{ c c c }
% Hyperparameters & Range  \\ \hline \hline 
% conv1-kernel-size & $\{1,2,\cdots,7\}$ \\ \hline  
% conv2-kernel-size & $\{1,2,\cdots,7\}$ \\ \hline  
% %& $\{1,2,\cdots,7\}$ \\ \hline 
% conv3-kernel-size & $\{1,2,3 \}$ \\ \hline 
% pooling1-size  & $\{1,2,3\}$ \\ \hline 
% pooling2-size & $\{1,2,3\}$ \\ \hline 
% pooling3-size & $\{1,2,\cdots, 6 \}$ \\ \hline 
% $\beta_1$ \& $\beta_2$ & $\{0 , 0.05 ,  \cdots, 1 \}$  \\ \hline 
% learning-rate & 1e-6 to 5 \\ \hline
% learning-rate-redeuction & \{1,2,3\} \\ \hline
% \makecell{training-iteration\\ (only for Setting A) } & $\{200,400, \cdots,3000\}$ \\ \hline
% \end{tabular}
% }
% \caption{Settings for CIFAR-10 experiments.}
% \end{table} 

% \begin{table}[H]
%     \centering
%     \begin{tabular}{c | c}
%         Training Iterations & \makecell{Number of \\ different configurations} \\ \hline \hline
%         263 & 12 \\
%         395 & 8 \\
%         592 & 5 \\
%         888 & 3 \\
%         1333 & 2 \\
%         2000 & 1 \\
%         3000 & 1 \\ \hline
%         395 & 8 \\
%         592 & 5 \\
%         888 & 3 \\
%         1333 & 2 \\
%         2000 & 1 \\
%         3000 & 1 \\ \hline
%         592 & 6 \\
%         888 & 4 \\
%         1333 & 2 \\
%         2000 & 1 \\
%         3000 & 1 \\ \hline
%         888 & 4 \\
%         1333 & 2 \\ 
%         2000 & 1 \\
%         3000 & 1 \\ \hline
%         1333 & 5 \\
%         2000 & 3 \\
%         3000 & 2 \\ \hline
%         2000 & 5 \\
%         3000 & 3 \\ \hline
%         3000 & 7 \\ \hline
%     \end{tabular}
%     \caption{The pattern of resource increase for Hyperband and CTUCB in Section \ref{sec:cifar}. The table represents the resource increase in the following way. The first row states that Hyperband and CTUCB first train 12 different neural networks, each with 263 training iterations; then the second row states that both algorithms then train 8 neural network each with 395 iterations; and so on. } 
%     \label{tab:cifar-resouce}
% \end{table}

% As shown in Figure \ref{fig:cnn-cifar}, our methods find good configurations faster than other methods most of the time.
% In particular, in Setting A, TUCB reaches 70\% accuracy using 30,400 iterations, while other methods on average require 42,800 iterations; in Setting B, TUCB reaches 70\% accuracy using 11,943 iterations, while other methods on average require 71,934 total iterations.\footnote{In our averages for Setting A, for methods that required over 45,000 iterations to reach 70\% accuracy, we simply denoted that they required 45,000 iterations. 
% In our averages for Setting B, for methods that required over 120,000 iterations to reach 70\% accuracy, we simply denoted that they required 120,000 iterations.} In addition, TUCB does not achieve above 0.754 accuracy after 45,000 iterations in Setting A, while CTUCB achieves above 0.76 accuracy within 45,000 iterations in Setting B. This shows that leveraging the training iterations as a special dimension can help increase the accuracy on an absolute scale. 





==> tex/inequality-wilson.tex <==
\subsection{Proof of (\ref{eq:point-scattering-1})} 
\label{app:point-scattering-1}

Consider the partition $ \mathcal{P}_T $ at time $T$. We label the regions of the partitions by $j = 1,2, \cdots, |\mathcal{P}_T|$. Let $t_{j,i}$ be the time when the $i$-th point in the $j$-th region in $\mathcal{P}_T$ being selected. Let $b_j$ be the number of points in region $j$. Since the partitions are nested, we have $1 + n_{t_{j,i} - 1}^0 (x_{t_{j,i}}) \ge i$ for all $i,j$. We have, for $T \ge 1$, 

\begin{align}
    \sum_{t=1}^T\frac{1}{1 + n_{t-1}^0 (x_t)} &= \sum_{j=1}^{|\mathcal{P}_T|}\sum_{i=1}^{b_j} \frac{1}{1 + n_{t_{j,i} - 1}^0 (x_{t_{j,i}}^0 )} \nonumber \\
    &\le \sum_{j=1}^{|\mathcal{P}_T|}\sum_{i=1}^{b_j} \frac{1}{i} \label{eq:ineq} \\
    &\le \sum_{j=1}^{|\mathcal{P}_T|} \left( 1 + \log b_j \right) \nonumber \\
    &= |\mathcal{P}_T| + \sum_{j=1}^{|\mathcal{P}_T|}  \log b_j \nonumber \\ 
    &= |\mathcal{P}_T| + \log  \prod_{j=1}^{|\mathcal{P}_T|} b_j \nonumber \\
    &\le |\mathcal{P}_T| + |\mathcal{P}_T| \log  \frac{T}{|\mathcal{P}_T|}. \label{eq:am-gm},
\end{align}
where (\ref{eq:ineq}) uses $1 + n_{t_{j,i} - 1}^0 (x_{t_{j,i}}) \ge i$ and (\ref{eq:am-gm}) uses AM-GM inequality and that $\sum_{j=1}^{|\mathcal{P}_T|} b_j = T$. 

\subsection{Proof of (\ref{eq:point-scattering-alpha})}
\label{app:point-scattering-alpha}

The idea is similar to that of (\ref{eq:point-scattering-1}). The key observation is stated in the first paragraph in Appendix \ref{app:point-scattering-1}. For $0< \alpha < 1$, 
\begin{align}
    \sum_{t=1}^T \left( \frac{1}{1 + n_{t-1}^0 (x_t)} \right)^{\alpha} &=  \sum_{j=1}^{|\mathcal{P}_T|}\sum_{i=1}^{b_j} \left( \frac{1}{1 + n_{t_{j,i}}^0 (x_{t_{j,i}}^0 )} \right)^\alpha \nonumber \\
    &\le \sum_{j=1}^{|\mathcal{P}_T|}\sum_{i=1}^{b_j} \frac{1}{i^\alpha} \nonumber \\
    &\le \sum_{j=1}^{|\mathcal{P}_T|} \frac{1}{1-\alpha} b_j^{1 - \alpha} \nonumber \\
    &\le \frac{1}{1 - \alpha} |\mathcal{P}_T|^\alpha T^{1 - \alpha} \label{eq:holder},
\end{align}

where (\ref{eq:holder}) is due to the H\"older's inequality and that $\sum_{j=1}^{|\mathcal{P}_T|} b_j = T$. 

==> tex/introduction.tex <==
% !TEX root = ../writeup.tex

\section{Introduction} \label{introduction}
The goal of many important real-world problems is to optimize an underlying function whose evaluation is expensive. Minimizing the number of times to query the underlying function is then desired. Problems of this kind include experimental design \citep{chaloner1995bayesian,srinivas2009gaussian,martinez2014bayesopt}, online recommendation \citep{ricci2015recommender}, data-efficient system control \citep{calandra2016bayesian, lizotte2007automatic, mukadam2017continuous}, and tuning neural network hyperparameters (kernel size, pooling size, learning rate and its decay rate). Tuning hyperparameters of neural networks is not simply a gradient-free optimization problem, since some hyperparameter settings are significantly more expensive than others to be evaluated. When the user can control the computational resources dedicated to the tuning, algorithms within the stochastic bandit framework should be leveraging this control to obtain cost-effective performance, as is also suggested in the Bayesian Optimization setting \citep{kandasamy2017multi, song2018general}.
%this becomes more complicated than a straightforward function evaluation scheme.
%Bayesian optimization techniques \citep{shahriari2016taking,snoek2012practical} and 
 %, since these methods try to locate the optimal value as quickly as possible by balancing exploration and exploitation. x

%Stochastic bandit algorithms %\textcolor{red}{Did Bubeck invent stochochastic bandit in 2012? The way you cite it makes it sound like he did. But I doubt it} 
%optimize an underlying payoff function efficiently by balancing exploitation and exploration. 
%\textcolor{red}{
A stochastic bandit problem assumes that payoffs are noisy and are drawn from a unchanging distribution. The study of stochastic bandit problems started with the discrete arm setting, where the agent is faced with a finite set of choices. %, where each choice has the same cost but potentially different rewards. 
Classic works on this problem date back to the Thompson Sampling problem \citep{thompson1933likelihood}, Gittins index \citep{gittins1979bandit}, and some Upper Confidence Bound (UCB) methods \citep{lai1985asymptotically, agrawal1995sample}. Common solutions to this problem include the $\epsilon$-greedy algorithms \citep{sutton1998introduction}, the UCB-based algorithms \citep{auer2002finite}, and the Thompson Sampling algorithms \citep{agrawal2012analysis}. These bandit strategies have led to powerful real-life applications. For example, Deep Q-Network \citep{mnih2015human} uses $\epsilon$-greedy for action exploration; and AlphaGO \citep{silver2016mastering} uses UCT \citep{kocsis2006bandit}, which is built on the UCB strategy, for action searching. %{\color{red} (UCB being a fairly complete solution  is a comment made by John Langford or Sebastien Bubeck. Well, I feel the same way on this, but still I'm not sure whether I should state that it is a relatively complete solution to this problem here - why would you do that? sounds like it's already solved, so why bother write this paper if it's solved?)}; 
One recent line of work on stochastic bandit problems considers the case where the arm space is infinite. In this setting, the arms are usually assumed to be in a subset of the Euclidean space (or a more general metric space), and the expected payoff function is assumed to be a function of the arms. 
Some works along this line model the expected payoff as a linear function of the arms \citep{auer2002using,dani2008stochastic,li2010contextual,abbasi2011improved,agrawal2013thompson, abeille2017linear}; some algorithms model the expected payoff as Gaussian processes over the arms \citep{srinivas2009gaussian,contal2014gaussian,de2012exponential,vazquez2007convergence}; some algorithms assume that the expected payoff is a Lipschitz function of the arms \citep{slivkins2011contextual, kleinberg2008multi,bubeck2011x}; and some assume locally H\"older payoffs on the real line \citep{auer2007improved}. When the arms are continuous and equipped with a metric, and the expected payoff is Lipschitz continuous in the arm space, we refer to the problem as a stochastic Lipschitz bandit problem. In addition, when the agent's decisions are made with the aid of contextual information, we refer to the problem as a contextual stochastic Lipschitz bandit problem. In this paper, we focus our study on the (contextual) stochastic Lipschitz bandit problems, and its application to neural network tuning. 
While our analysis focuses on the case of Lipschitz expected payoffs, our empirical results demonstrate that our methods can adapt to the landscape of the payoff and leverage properties other than Lipschitzness. This means our methods in practice have much better performance than analyses for Lipschitz bandit problems suggest. 
Few of the methods listed above consider computational resources as part of the algorithm, even though it is important for neural network tuning and other important problems. 
%(Hyperband considers computational resource and is listed in the related work section below. So perhaps it's better not to make this statement here. But the statement is correct - none of the above methods use computational resources. So it's a relatively minor concern. Is this better? ) }
%This means that the methods is when Lipschitzness is replaced 

%For a more complete review, please refer to \citep{bubeck2012regret}. 

%{\color{red} While the (contextual) Zooming bandit algorithm serves as an solution to the (contextual) stochastic Lipschitz bandit problem, they suffer from practical inefficiency (see the Related Work section). 
Neural network tuning is challenging, and in recent years, the best performance has relied heavily on human tuning of the network's hyperparameters. 
%While neural networks have advanced amazing real-world applications, good performance is usually built on top of heavy human effort. Since stochastic bandit algorithms can be used to optimize black-box function whose evaluation is expensive, we apply our stochastic Lipschitz bandit algorithms to neural network tuning. 
%For the problem of training neural networks, 
Given a training and validation set, the validation performance metric (e.g. validation accuracy) of the neural network can be viewed as a noisy function (payoff) of hyperparameters (arms), which include the architecture of the network, the learning rate, initialization, the number of training iterations, etc. This turns a neural network tuning problem into a stochastic bandit problem. The arms have different costs: if we train only for a small amount of iterations, we use less resources. Training for a small amount of iterations is often useful to judge initial conditions and architecture. Ideally, the method should be able to choose how long (how many iterations) to train in order to balance between exploration, exploitation, and cost of evaluation. %\textcolor{red}{
As shown in Section \ref{sec:exp}, our methods balance between exploration, exploitation, and cost of evaluation for the problem of neural network tuning. 
%(I'm a bit confused by the few sentences before this. It sounds like a general comment to this problem, and it sounds like a comment to our methods as well. So I tried to clarify it a bit. )}
%\textcolor{red}{In addition, training cost can be saved by starting with small training resource budget and progressively increase it.}
%In this problem, the hyperparameter configurations ( e.g. learning rate, number of hidden neurons, etc.) are viewed as arms, and the performance metric (e.g. validation accuracy) is viewed as payoffs.
%Based on empirical results on tuning neural networks for benchmark datasets, our methods tend to be more efficient and/or effective than the existing state-of-the-art tuning methods. (See related work.)


%In this paper, we develop a novel (contextual) stochastic Lipschitz bandit algorithm and apply it to tuning neural networks. Our approaches are efficient and easy-to-implement; we also provide a read-to-go implementation of stochastic Lipschitz bandit algorithms. Real-world empirical studies demonstrate the strength of our method in complex tasks such as neural network tuning. 
%I think you need a better transition here. What is your key insight? Is it the adaptive partition? Probably not. It is that viewing the resource dimension as an extra special dimension helped? See Regina's notes on how to write an abstract. 

Our proposed algorithm, (Contextual) PartitionUCB, maintains a finite partition of the (context-)arm space and uses an Upper Confidence Bound strategy \citep{auer2002finite}, as if the partition represents a finite set of (context-)arms. As we observe more data, the partition grows finer. To better deploy (Contextual)  PartitionUCB to problems such as neural network tuning, we provide fast implementations using regression trees, since a regression tree corresponds to a partition. We show empirically that our proposed tuning methods outperform existing state-of-the-art on benchmark datasets.  %Since the hyperparameter space of a neural network
In summary, our contributions are threefold: 
%\begin{enumerate}
\textbf{1)} we develop a novel stochastic Lipschitz bandit algorithm \textit{PartitionUCB} and its contextual counterpart \textit{Contextual PartitionUCB}. For compact domains in $\mathbb{R}^d$, both algorithms exhibit a $\mathcal{\tilde{O}} (T^{\frac{d+1}{d+2}})$ regret bound with high probability; 
\textbf{2)} we develop \textit{TreeUCB (TUCB)} and \textit{Contextual TreeUCB  (CTUCB)} as fast implementations of \textit{PartitionUCB} and \textit{Contextual PartitionUCB}. We apply TUCB and CTUCB to tuning neural networks. They can achieve a satisfactory level of accuracy as the average of existing state-of-the-art approaches while saving over 50\% resource (e.g. time, total training iterations) on the MNIST dataset \citep{lecun1998mnist}, the SVHN dataset  \citep{netzer2011reading} dataset and the CIFAR-10 dataset \citep{krizhevsky2012imagenet}; \textbf{3)} we introduce the ``so-called'' point scattering inequality for as a technical tool to analyze the regret bound, which can be used within and beyond the stochastic bandit problems. 
%\end{enumerate} 



%{\color{red} The rest of the paper is developed as follows: we first state related workd below; then we introduce the \textit{PartitionUCB} algorithm and \textit{Contextual PartitionUCB} algorithm in Section \ref{algorithm-non-contextual} }



%The problem of tuning a neural network is particularly challenging because we want to minimize not only the number of queries made, but also computing resources used. For the problem of training neural networks, given a training set, the validation accuracy of the neural network at a fixed number of iterations can be viewed as a function of hyperparameters: the architecture, the learning rate, the dropout rate \cihttps://www.overleaf.com/project/5c0a0db390a3462b80c6ef01te{srivastava2014dropout} and so on. We want to locate the best hyperparameter configuration so that the validation accuracy is maximized. 

%{\color{red}One approach to limit training resources is to leverage training resources as a special hyperparameter dimension for neural networks. }
%the number of training iterations is a special dimension for neural networks. 
%For example, the number of epochs (iterations), as a training resource itself, can be considered as a special dimension of a neural network.  Since the neural network converges over epochs, validation accuracy at different iterations can estimate the performance of a neural network at different levels of number of epochs. The performance at a smaller epochs can potentially help infer the performance at a larger epochs while saving computing resources. 

%In this paper, we propose a bandit-based upper confidence bound algorithm for tuning neural networks. 


%Behind the fascinating performance of neural networks is usually a huge effort of manual tuning. However, machine learning should not depend on humans so much. Therefore we propose algorithms TreeUCB (TUCB, Algorithm \ref{alg:tucb}) and Contextual TreeUCB (CTUCB, Algorithm \ref{alg:ctucb}) based on bandit algorithms with theoretical guarantees PartitionUCB (Algorithm \ref{alg:bandit}) and Contextual-PartitionUCB (Algorithm \ref{alg:contextual-bandit}). We make sure that the algorithms save resources such as training epochs to a large extent. \\
\vspace{0.5cm}
\noindent 
\textbf{Related works: } From a bandit perspective, the closest works are the Zooming bandit algorithm (and the contextual Zooming bandit algorithm) \citep{slivkins2011contextual, kleinberg2008multi} and the HOO algorithm \citep{bubeck2011x}, which inspired our work. Both the Zooming bandit algorithm and the HOO algorithm have excellent theoretical analyses, but suffer from practical inefficiency. 
%Compared to the Zooming bandit algorithm, it does not require a covering oracle and the doubling trick \citep{bubeck2011x}. 
The Zooming bandit algorithm (and the contextual Zooming bandit algorithm) keeps a cover of the arm space. As the Zooming bandit runs, some subsets in the cover shrink, resulting in some points of the arm space becoming uncovered. Once this happens, the algorithm needs to introduce new subsets of arms to maintain the cover. The operation of checking whether each arm is covered can be expensive and hard-to-implement in practice. 
The HOO algorithm does not require Zooming bandit's covering oracle, but it is non-contextual. This makes it less general than the Contextual PartitionUCB algorithm. In addition, it requires a fine discretization of the arm space to start with. This initialization requirement makes HOO impractical, since problems like tuning neural networks can have arm spaces with millions of points in discrete spaces or infinite points in a parameter space. 
% is more general than HOO since HOO is non-contextual.}
%hierarchically arranging a large number of the subsets of the arms space to start with. More specifically, HOO discretizes the arm space and puts the entire discretized arm space on level 1 and the two disjoint half subspaces on level 2. HOO then recursively evenly divides the subspaces and arrange the halves on the next level until there are only singletons. 
 %In fact, as we will see in Section \ref{experiment}, a multi-layer perceptron \citep{rumelhart1985learning} with only one hidden layer can have more than one million possible hyperparameter configurations. %In addition, compared to the HOO algorithm, our regret bound is a high probability bound instead of a bound of the expected regret. 
%Since our method maintains a partition of the space, we can make use of fast implementations of regression trees \citep{}. 
The practical efficiency of our method is partially a result of maintaining a careful partition of the space. This allows us to use a fast implementation of regression trees \citep{geurts2006extremely}. %{\color{red} The tree implementations are called the \textit{Tree-UCB (TUCB)} and the \textit{Contextual TreeUCB (CTUCB)} algorithms.  }
%it does not require arranging a large amount of subsets of the candidates in a hierarchical fashion to start, it also comes with a high probability bound instead of just a bound on the expectation. 
%As a non-parametric method with only a Lipschitz assumption on the underlying function, it is more flexible than linear methods \citep{chu2011contextual, auer2002using, abbasi2011improved}.  

 Empirical results on tuning neural networks for the MNIST dataset \citep{lecun1998mnist}, the SVHN dataset \citep{netzer2011reading} dataset and the CIFAR-10 dataset \citep{krizhevsky2012imagenet}, indicate that our methods tend to be more efficient and/or effective than 1) the state-of-the-art Bayesian optimization methods: the SPEARMINT package \citep{snoek2012practical} which integrates several Bayesian optimization methods \citep{swersky2013multi, bergstra2011algorithms, snoek2014input, snoek2013bayesian, gelbart2014bayesian}, the TPE algorithm \citep{bergstra2011algorithms} and the SMAC algorithm \citep{hutter2011sequential}; and 2) methods that focus explicitly on tuning neural networks: Hyperband algorithm \citep{li2016hyperband} (and SuccessiveHalving algorithm \citep{jamieson2016non}), the Harmonica algorithm \citep{hazan2017hyperparameter}, and random search \citep{bergstra2012random}. %\textcolor{red}{
As suggested by the results in this paper, common bandit algorithms, such as UCB algorithms, can be competitive with the state-of-the-art methods for neural network tuning. 



In what's following, we begin by recapping the classic UCB1 algorithm \citep{auer2002finite} for stochastic bandit problem and introduce the point scattering inequality. We then introduce the algorithms. We finally deploy the empirical version of the algorithms to the task of neural network tuning, and show empirical evidence of the strength of the algorithms. 
 %this language needs to be fixed but I'm out of time.
% }
%Also, the practical efficiency of our method helps it to naturally surpass a class of methods based on Gaussian processes, such as GP-UCB \citep{srinivas2009gaussian, krause2011contextual}, GP-MI \citep{contal2014gaussian} and GP-EI \citep{jones1998efficient}, since the computation of the Gram matrix can be expensive. 
%%We studied the performance of TUCB and CTUCB on the MNIST dataset \citep{lecun1998mnist} and the SVHN dataset \citep{netzer2011reading} against two comparison schemes. TUCB and CTUCB tend to be more efficient and/or effective than the state-of-the-art Bayesian optimization methods: the SPEARMINT package \citep{snoek2012practical} which integrates several Bayesian optimization methods \citep{swersky2013multi, bergstra2011algorithms, snoek2014input, snoek2013bayesian, gelbart2014bayesian}, the TPE algorithm \citep{bergstra2011algorithms} and the SMAC algorithm \citep{hutter2011sequential}. 
%%There are also methods that focus explicitly on tuning neural networks, inluding the Hyperband algorithm \citep{li2016hyperband} (and SuccessiveHalving algorithm \citep{jamieson2016non}), the Harmonica algorithm \citep{hazan2017hyperparameter}, and random search \citep{bergstra2012random}. The experimental results show that the proposed method outperforms the state-of-the-art methods. 

%In this paper, we propose and analyze a practically efficient algorithm for the Lipschitz X-armed bandit setting \citep{bubeck2011x,bubeck2009online}. The term X-armed bandit is used when the arm space is Lebesgue measurable, or from practical viewpoint, some dimensions of the arm space (function input space) are numeric while the rest are finite categorical. The term Lipschitz implies the Lipschitz continuity assumption of the underlying function. In order to properly define Lipschitz continuity for the categorical features, we embed those dimensions onto a simplex or a hypercube. Many previous works \citep{auer2002using,chu2011contextual,agrawal2013thompson} handles discrete arm space but not continuous arm space. On the other hand, the algorithms that handles continuous arm space \citep{benassi2011robust,contal2014gaussian,krause2011contextual,abbasi2011improved, dani2008stochastic} are inherently slow. Specifically, in principle at every iteration, \citep{benassi2011robust,contal2014gaussian,krause2011contextual} requires constructing (and inverting) the kernel matrix; \citep{abbasi2011improved, dani2008stochastic} requires solving a complex optimization problem that is NP-hard for certain norm choices. \\\\ %\textcolor{red}{Some more literature review on recent ``scalable bandits'' goes here. } \\\\
%\textbf{Related work:} while the algorithm is related to the Zooming bandit algorithm \citep{kleinberg2008multi, slivkins2011contextual} and the Hierarchical Optimistic Optimization (HOO) algorithm \citep{bubeck2011x}. The algorithm is mostly related to XXX. Nonetheless, compared to the Zooming bandit algorithm and HOO, , we provide an high probability bound on the cumulative (pseudo-)regret instead of a bound on the expected (pseudo-)regret. \\\\
%\noindent
%In this paper, we propose to use regression trees coupled with the Upper Confidence Bound heuristic to stress the problems. This approach is 1) scalable as regression trees are scalable \citep{geurts2006extremely}, 2) automatically handled the X-armed space. We assume that the underlying function is Lipschitz continuous. This setting is commonly referred to as the Lipschitz bandit problem \citep{magureanu2014lipschitz,kleinberg2008multi}. This assumption is weaker than linearity or Gaussian process with a smooth (differentiable) kernel, which is often seen in the literature. The rest of this paper is developed in the following way. In section \ref{algorithm}, we first formally state the problem and state the algorithm. In section \ref{analysis}, we provide a high probability regret bound for the algorithm. In section \ref{experiment}, we give an extension to incorporate context information under mild assumptions. We also propose a practical implementation and study empirically the performance in terms of both regret and computational time. \\

